Byzantine Consensus in the Random Asynchronous Model

We propose a novel relaxation of the classic asynchronous network model, called the random asynchronous model, which removes adversarial message scheduling while preserving unbounded message delays and Byzantine faults. Instead of an adversary dictating message order, delivery follows a random schedule. We analyze Byzantine consensus at different resilience thresholds ($n=3f+1$, $n=2f+1$, and $n=f+2$) and show that our relaxation allows consensus with probabilistic guarantees which are impossible in the standard asynchronous model or even the partially synchronous model. We complement these protocols with corresponding impossibility results, establishing the limits of consensus in the random asynchronous model.

==> sections/bullshark.tex <==
\section{Practical Consensus Protocols in the \model}
\label{sec:practical}

The algorithms in the previous sections are simple and easy to understand, but they are not practical for modern applications such as blockchain. Instead, such applications increasingly use DAG-based consensus protocols~\cite{mysticeti, bullshark, narwhal}. 

Here, we briefly describe how to obtain a practical DAG-based deterministic consensus protocol for the \model.

One such protocol can be easily derived from the partially synchronous version of Bullshark~\cite{PSBullshark}, by removing timeouts. The original algorithm uses timeouts to ensure liveness, as follows: 
\begin{enumerate}
    \item In even rounds, upon receiving $n-f$ messages that do not contain a message from the round's anchor (leader), a correct process additionally waits for a message from the leader, or a timeout.
    \item In odd rounds, correct processes wait for $f+1$ messages that vote for the previous round's anchor, or for $n-f$ messages that do not vote for the anchor, or for a timeout.
\end{enumerate} 

Without the timeouts, the original algorithm would not satisfy liveness in the partially synchronous model, since the adversary can always delay messages such that, for example, no correct process ever receives the anchor message of any round among the first $n-f$ messages, which would prevent progress. Note that, even with the timeout, it is possible, before GST, for some anchors not to be committed.

However, in the \model, we can remove the timeouts, thus obtaining a deterministic asynchronous consensus protocol, and still guarantee liveness (with probability 1). 

\alberto{
We can discuss the composition of \model with synchrony to obtain a "partial random async model", and indicate that they inherit the best of both worlds
}



==> sections/old/intro.tex <==
\section{Introduction}\label{sec:intro}

Most current message-passing distributed algorithms assume model in which the adversary, in addition to being able to corrupt a subset of the participants, also has control over the network. More precisely, the standard asynchronous model typically assumes that the adversary controls the \textit{message schedule}, i.e., the order in which messages are delivered.

This model is a good worst-case model to design algorithms against. It captures the scenario in which the network behaves adversarially, either by bad luck, or by actual influence of a malicious adversary over the network.

However, in this paper, we argue that the standard model is too pessimistic. We believe that it is not realistic to assume that the adversary has control over the network. Instead, we propose the more realistic assumption that the network is independent of the adversary's influence, and is instead random. In more precise terms, in an asynchronous random network, every process is equally likely to have its message delivered next.

As we show in the paper this has several interesting theoretical and practical implications for the consensus problem. All of our results assume full asynchrony and deterministic processes. By deterministic here we mean that correct processes do not have access to sources of randomness. Such deterministic asynchronous consensus (DAC) protocols are highly desirable in practice, since they do not rely on timeouts, nor on expensive cryptographic sources of randomness.

We first show that in a random network, the consensus problem can be solved deterministically in full asynchrony, with both crash faults and Byzantine faults, circumventing the well-known FLP impossibility result~\cite{FLP}.  Our first protocol ensures safety (agreement and validity) at all times, and termination with probability 1. 

Secondly, we show that a with-high-probability-safety (WHPS) version of Byzantine consensus can be solved in the fair model, even if $n=2f+1$. WHPS here means that agreement and validity are ensured with high probability, and termination is ensured deterministically.

Finally, we show that by relaxing the problem even further, and ensuring only weak or external validity whp, as well as whp agreement and deterministic termination, the Byzantine consensus problem can be solved in the fair network model even if $n \leq 2f$.

Intuitively, the eventual fairness model enables these protocols because the randomness of the network ensures that an infinitely long bad schedule, i.e. one that would prevent termination or break safety, has probability $0$, or negligible probability, respectively. To see this, consider a DAC protocol $\mathcal{P}$ that is indulgent~\cite{indulgent-algs} towards the randomness property, i.e., $\mathcal{P}$ ensures safety even if the fairness property does not hold---we will present such protocols in \Cref{sec:warmup}. $\mathcal{P}$ proceeds in rounds: in each round correct processes attempt to agree on a single value. If in some good round, all processes receive messages from all other correct processes, then they can agree and decide. Many consensus protocols of this form exist, but in the standard asynchronous model, the adversary can choose a schedule that prevents good rounds from ever occurring. However, in the random network model the adversary no longer has this option. Since the probability of a good round is nonzero, the probability of an infinite sequence of bad rounds is zero---in other words, termination is guaranteed with probability 1. 

Similar assumptions to our random network have been explored by previous work. In message passing, the seminal paper of Bracha and Toueg~\cite{BrachaT85} defines the fair scheduler, which ensures that in each message round, there is a constant non-zero probability that each correct process receives messages from the same set of correct processes. It then proposes deterministic asynchronous binary consensus protocols for the crash-fault and Byzantine-fault models under the fair scheduler assumption. In shared memory, Aspnes~\cite{Aspnes02} defines noisy scheduling, in which the adversary may chose the schedule, but that adversarial schedule is perturbed randomly. He shows that with such a noisy schedule, deterministic asynchronous consensus is achievable. Also in shared memory, previous work introduce a \textit{stochastic scheduler}~\cite{AlistarhSV15,AlistarhCS16}, which schedules shared memory steps randomly. This line of work shows that many lock-free algorithms are essentially wait-free when run against a stochastic scheduler, because the schedules that would break wait-freedom have negligible probability. 

Here is a summary of our results:

\begin{table}[ht]
  \centering  % Center the table

  \begin{tabular}{ccc} % Define the table with 3 centered columns (ccc)
    \toprule  % Top rule using booktabs
    Resilience & Positive Result & Negative Result \\
    \midrule  % Mid rule using booktabs
    $n = 3f + 1$ & Det. strong safety \& P1 termination & Det. strong safety \& det. termination \\
    $n = 2f + 1$ & Whp strong safety \& det. termination & P1 safety \& det. termination \\
    $n = f + 2$ & Whp weak safety \& det. termination & P1 weak safety \& det. termination \\
    \bottomrule  % Bottom rule using booktabs
  \end{tabular}
  \caption{Results in this paper for Byzantine consensus. 
  \textit{Det.} means ``deterministic", \textit{P1} mea ns ``with probability 1'', and \textit{whp} means ``with high probability". Strong safety means agreement and strong validity. Weak safety means agreement and weak validity.
  }  % Add a caption
\end{table}


==> sections/old/warmup.tex <==
\section{Deterministic safety, termination with probability 1}
\label{sec:warmup}

We provide in this section algorithms for crash-tolerant binary consensus and strong Byzantine consensus, which satisfy all of their safety properties deterministically (i.e., in every execution), and termination with probability $1$. Both algorithms share the same skeleton, shown in \Cref{alg:skeleton}. 

\Cref{alg:skeleton} relies on a novel variant of the adopt-commit (AC) object~\cite{ac1, ac2}, which we call \textit{fair adopt-commit} (FAC). The specification of the FAC object is given in Module~\ref{mod:fac}. The FAC object differs with respect to the standard AC object only in its \textit{fairness} property, which informally ensures that with at least some constant nonzero probability, all correct processes agree in their output from the FAC object, even if they do not have the same input.

\begin{module}
\caption{Crash-Tolerant Fair Adopt-Commit (FAC)}
\label{mod:fac}
\begin{algorithmic}[1]

\Statex \textbf{Interface}:
\Statex \hskip1em \textsc{Propose}$(v)$, where $v$ is a value. Returns $\{\langle \textsc{Grade}, v' \rangle\}$, where $\textsc{Grade} \in \{\textsc{Commit}, \textsc{Adopt}\}$ and $v'$ is \hphantom{mmm}a value.


\bigskip
\Statex \textbf{Properties:}
\Statex \hskip1em \emph{Integrity:} If a process returns $(\cdot, v)$, then $v$ was proposed by some process.
\smallskip 

\Statex \hskip1em \emph{Strong validity:} If all correct processes propose the same value $v$ and a correct process returns a pair \hphantom{mmm}$\langle \textsc{Grade}, v' \rangle$, then $\textsc{Grade} = \textsc{Commit}$ and $v' = v$.

\smallskip 
\Statex \hskip1em \emph{Consistency:} If any correct process returns  $\langle \textsc{Commit}, v' \rangle$, then no correct process returns $(\cdot, v' \ne v)$.

\smallskip 
\Statex \hskip1em \emph{Termination:} If all correct processes propose, then every correct process eventually returns.

\smallskip
\Statex \hskip1em \textit{Fairness:} There exists a constant $P>0$ such that, with probability at least $P$, all correct process that \hphantom{mmm}return, return the same value $v$ (possibly with different \textsc{Grade}s).

\end{algorithmic}
\end{module}

\Cref{alg:skeleton} proceeds in rounds: in each round, processes attempt to decide using a fresh FAC object. The fairness property of the FAC objects ensures that, with probability 1, correct processes eventually have the same estimate and thus, by the strong validity of FAC, all correct processes eventually return \textsc{Commit} and decide. The specific implementation of the AC object differs between the crash-only and Byzantine cases.

\begin{algorithm}
\caption{Skeleton consensus algorithm: pseudocode at process $i$}
\label{alg:skeleton}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip1em \textsf{FAC}[$0, \cdots$], an infinite array of FAC objects
\bigskip

\State \textbf{procedure }\textsc{Propose}$(v_i)$: 
\BlueComment{$v_i \in \{0,1\}$}
\State \hskip1em $est_i \gets v_i$
\State \hskip1em $r_i \gets 0$
\State \hskip1em \textbf{while} \textsf{true}:
\State \hskip2em \textbf{switch} \textsf{FAC}[$r_i$].\textsc{Propose}$(est_i)$:
\State \hskip3em \textbf{case} $\langle \textsc{Commit}, v \rangle$: \textsf{decide}$(v)$\label{line:skeleton-decide}
\BlueComment{Only once}
\State \hskip3em \textbf{case} $\langle \textsc{Adopt}, v \rangle$: $est_i \gets v$
\State \hskip2em $r_i \gets r_i + 1$
\end{algorithmic}
\end{algorithm}

\subsection{Crash Faults}

\Cref{alg:aac-crash} is adapted from~\cite{book}. It gives an implementation of crash-fault tolerant FAC under the assumption that $n=2f+1$.

The algorithm consists of two
phases. In the first phase, every correct process proposes a value by sending it to
all processes. Then it receives proposals from
a quorum of processes. If a process observes that all responses contain the same
phase-one proposal value then it proposes that value for the second phase. If a process does not obtain a unanimous set of proposals in the first phase, the process simply proposes $\bot$ for the second phase.

Note that as a result of this procedure, if two processes propose a value different from $\bot$ for the second phase, they propose exactly the same value.
Let this value be called $v*$.

The purpose of the second phase is to verify if $v*$
was also observed by enough other processes.
After a process receives $n-f$ phase-two messages, it checks if more than $f$ phase-two proposals are equal to $v*$, and may commit this value if there are enough of them. A process adopts $v*$ if it receives $v*$ in the second phase, but is unable to collect enough $v*$ values to decide. Finally, it is possible that a process does not receive $v*$ in the second phase (either because no such value was found in phase one or simply because it has received only $\bot$ in phase two); in this case the process adopts the fist value it received in phase one (we call this the \textit{first-seen-value (FSV) adopt rule}).

Except for the FSV adopt rule, the algorithm is a standard adopt-commit protocol. The additional fairness property comes from the FSV rule. In the fair model, the event that all correct processes receive the same value $v$ first has non-zero probability \lef{because they will all receive the same proposal from the same proposer?}. Thus, if the processes cannot deterministically choose the same value, the FSV rule gives them a non-zero probability to converge.  

\begin{algorithm}
\caption{Crash-fault tolerant FAC: pseudocode at process $i$}
\label{alg:aac-crash}
\begin{algorithmic} [1]
\State \textbf{procedure} \textsc{Propose}$(v)$:
\State \hskip1em Send $\langle \textsc{Init}, v \rangle$ to all processes\label{line:fac-crash-init}
\BlueComment{Phase 1}
\State \hskip1em Wait for $n-f$ $\langle \textsc{Init}, \_ \rangle$ messages\label{line:fac-crash-wait-init}
\State \hskip1em \textbf{if} $\exists\, v^*$ such that I received $>n/2$ $\langle \textsc{Init}, v^* \rangle$ messages:\label{line:fac-crash-if-init}
\State \hskip2em $proposal \gets v^*$ 
\State \hskip1em \textbf{else}:
\State \hskip2em $proposal \gets \bot$ 
\medskip
\State \hskip1em Send $\langle \textsc{Echo}, proposal \rangle$ to all processes
\BlueComment{Phase 2}\label{line:fac-crash-send-echo}
\State \hskip1em Wait for $n-f$ $\langle \textsc{Echo}, \_ \rangle$ messages\label{line:fac-crash-wait-echo}
\State \hskip1em \textbf{if} $\exists\, v^* \ne \bot$ such that I received $\geq f+1$ $\langle \textsc{Echo}, v^* \rangle$ messages:
\State \hskip2em \textbf{return} $\langle \textsc{Commit}, v^* \rangle$\label{line:fac-crash-commit}
\State \hskip1em \textbf{else if} $\exists\, v^* \ne \bot$ such that I received $\geq 1$ $\langle \textsc{Echo}, v^* \rangle$ messages:
\State \hskip2em \textbf{return} $\langle \textsc{Adopt}, v^* \rangle$\label{line:fac-crash-adopt-det}
\State \hskip1em \textbf{else}:
\State \hskip2em $v^* \gets$ value in first \textsc{Init} message I received\label{line:fac-crash-adopt-rand}
\State \hskip2em \textbf{return} $\langle \textsc{Adopt}, v^* \rangle$ 
\end{algorithmic}
\end{algorithm}


\subsection{Byzantine Faults}

\Cref{alg:aac-byz} is adapted from Bracha and Toueg~\cite{BrachaT85}. It gives an implementation of Byzantine fault tolerant FAC under the assumption that $n=3f+1$.

There are two types of messages: initial and echo. A process sends to all the processes an initial message with its name and its value. Upon receiving an initial message, every process echoes it back to all the processes. Process $p$ \textit{accepts} a message with value $v$ from process $q$ if it receives more than $(n + f)/2$ messages of the form $(echo, q, v)$. 

Process $p$ waits until it has accepted values from $n-f$ senders. If $p$ has accepted more than $(n+f)/2$ messages with the same value $v$, $p$ may commit $v$. Otherwise, $p$ adopts the majority value.

The main intuition here is that the fair model ensures there is a non-zero probability that every correct process hears from every other correct process first, before any potential messages from faulty processes. In this case, correct processes will converge on (adopt) the same value. Thus the fairness property is ensured. \lef{Basically instead of hoping the random coin will give the same value to everyone we hope the network will deliver the same value to everyone? Would this explanation make it more intuitive on why it works?}

\begin{algorithm}
\caption{Byzantine-fault tolerant FAC: pseudocode at process $i$}
\label{alg:aac-byz}
\begin{algorithmic} [1]
\State \textbf{Local variables}:
\State \hskip1em $echo\_count[0..1]$, array initialized to $\{0,0\}$
\State \hskip1em $accepted\_count[0..1]$, array initialized to  $\{0,0\}$

\smallskip
\State \textbf{Message format}:
\State \hskip1em $type \in \{\textsc{Init}, \textsc{Echo}\}$
\State \hskip1em $origin \in \Pi$
\State \hskip1em $value$

\bigskip
\State \textbf{procedure} \textsc{Propose}$(v)$:
\State \hskip1em Send $\langle \textsc{Init}, i, v \rangle$ to all processes
\State \hskip1em \textbf{while} $accepted\_count[0] + accepted\_count[1] < n-f$:
\State \hskip2em $msg \gets \textsc{Receive}()$
\State \hskip2em \textbf{if} this is the first message from the sender with these values of $msg.type$ and  $msg.origin$:
\State \hskip3em \textbf{if} $msg.type$ is \textsc{Init}:
\State \hskip4em Send $\langle \textsc{Echo}, msg.origin, msg.value \rangle$ to all processes
\State \hskip3em \textbf{else}: \BlueComment{Echo}
\State \hskip4em $echo\_count[msg.origin][msg.value] += 1$
\State \hskip4em \textbf{if} $echo\_count[msg.origin][msg.value] \geq 2f + 1$:
\State \hskip5em $accepted\_count[msg.value] += 1$
\State \hskip1em \textbf{if} $accepted\_count[0] < accepted\_count[1]$: $value \gets 1$
\State \hskip1em \textbf{else}: $value \gets 0$
\State \hskip1em \textbf{if} $\exists\, v^*$ such that $accepted\_count[v] \geq 2f+1$:
\State \hskip2em return $\langle \textsc{Commit}, v^* \rangle$
\State \hskip1em \textbf{else}:
\State \hskip2em return $\langle \textsc{Adopt}, value \rangle$
\end{algorithmic}
\end{algorithm}
